The $\mathbb C$-motivic Adams-Novikov spectral sequence for topological modular forms

We analyze the $\mathbb{C}$-motivic (and classical) Adams-Novikov spectral sequence for the $\mathbb{C}$-motivic modular forms spectrum $\mathit{mmf}$ (and for the classical topological modular forms spectrum $\mathit{tmf}$). We primarily use purely algebraic techniques, with a few exceptions. Along the way, we settle a previously unresolved detail about the multiplicative structure of the homotopy groups of $\mathit{tmf}$.

==> leftovers.tex <==
\subsection{Leftovers}




We briefly summarize the question. For more details, see \cite[Def. 9.22, Prop. 9.35]{BR21}.

Consider ASS(tmf).
Let $\nu_2,\nu_4, \nu_6, D_4$ be Adams classes detected by $\Delta^2 h_2,  \Delta^4 h_2, \Delta^6 h_2$ and $2\Delta^4$ respectively. The ambiguity allows us to choose $\nu_4$ and $\nu_6$ such that 
\begin{equation}
\label{eq:definingrelation}
	\nu_2\nu_4=3\nu\nu_6, \text{ and } \nu D_4=2\nu_4.
\end{equation}
Let $M$ be a class detected by $\Delta^8$ and let $\nu$ be the Hurewicz image of the Hopf map. There is a relation
$$\nu_4\nu_6=s\nu\nu_2M.$$ Here the number $s$ is determined as long as we require the relations in (\ref{eq:definingrelation}), but it cannot be decided whether it is +1 or -1. In particular, by \cite{BR21}, the choices of $\nu_2$ and $\nu_4$ does not matter as long as the equations in (\ref{eq:definingrelation}) are satisfied.
 

\begin{thm}
Choose homotopy elements $\nu$, $\nu_2$, $\nu_4$, $\nu_6$ and $M$ as described above. There is a relation:
$$\nu_4\nu_6=-\nu\nu_2M.$$ 
\end{thm}

\begin{proof}
In the $E_\infty$ page of mANSS(mmf), $\Delta^{2n}h_2$ is a generator of $\mathbb Z/4.$ In other words, for example, when we choose $\nu_2$ to be a class detected by $\Delta^2h_2$, the ambiguity is between $\nu_2$ and  $5\nu_2$, and $-\nu_2$ (or $3\nu_2$) is detected by a different class $3\Delta^2h_2$.
In order to have $\nu_2\nu_4=3\nu\nu_6$, we choose $\nu_2,\nu_4, \nu_6$ to be elements detected by $\Delta^2 h_2,\Delta^4 h_2, 3\Delta^6 h_2.$

We the cofiber of $\tau$ method to detect the sign. Consider the elements 
$\tau\bar\kappa \nu_4 \nu_6$ and $\tau\bar\kappa \nu \nu_2M$ which are $\tau$-torsion.
The connecting homomorphism determines a map on homotopy groups 
$$\pi_{**}\mathrm{mmf}/\tau\to \pi_{*-1,*+1}\mathrm{mmf}.$$
Since the map is a $\pi_{**}\mathrm{mmf}$-module map,
by the differential 
$d_5(\Delta)=\tau^2 h_2 g$, we have the assignments
\begin{align*}
	\Delta^5\cdot \nu_6&\mapsto \tau\bar\kappa \nu_4 \cdot \nu_6,\\
\Delta\cdot \nu_2M & \mapsto \tau\bar\kappa\nu \cdot \nu_2M.
\end{align*}
Here $\Delta^5$ and $\Delta$ are homotopy elements in $\pi_{**}\mathrm{mmf}/\tau$ detected by the corresponding mANSS elements in the bottom cell. By our choice of $\nu_6$, we have $\Delta^5\cdot \nu_6 = 3 \Delta\cdot \nu_2M \in \pi_{**}\mathrm{mmf}/\tau.$ Thus in $\pi_{**}\mathrm{mmf}$, we have 
$$ \tau\bar\kappa \nu_4 \cdot \nu_6 = 3 \tau\bar\kappa\nu \cdot \nu_2M = -\tau\bar\kappa\nu \cdot \nu_2M.$$
\end{proof}

\subsection{Leftovers}

We choose $\Delta$ to have the property that the mANSS differential
$d_5(\Delta)$ equals $\tau^2 h_2 g$.  Other choices of $\Delta$ may lead
to the conclusion that $d_5(\Delta)$ equals $3 \tau^2 h_2 g$.
This choice is not necessarily compatible with the choice of 
edge homomorphism in \cite{BR21}.
However, this possible discrepancy is irrelevant for the relations
that we are studying.  
	




For our purposes, $\nu$ can be chosen to be an arbitrary generator of
the group $\pi_{3,2} \mmf$ of order $8$.  
For simplicity, we can choose $\nu$ to agree
with the definition in \cite{BR21}.
We also need to know the detecting element for $\nu$ in the
mANSS $E_\infty$-page.  The choice of $\nu$ as a generator implies
that it is detected by either $h_2$ or $-h_2$.

In fact, when defining generators of the mANSS $E_2$-page, 
$h_2$ is a choice of generator for the group $\Z/4$ in degree $(3,1,2)$.
This choice is expressed in the algebraic Novikov spectral sequence
by the presence of $h_0 h_2$ in higher algebraic Novikov filtration.
For convenience, we choose $h_2$ to be the element that detects $\nu$.

Similarly to $h_2$, there is also a choice of $\Delta$ when defining
mANSS $E_2$-page generators.  This is expressed by the presence of the 
elements $\Delta h_0^k$ in higher algebraic Novikov filtration.
For convenience, we choose $\Delta$ such that the 
Adams-Novikov differential $d_5(\Delta)$ equals $\tau^2 h_2 g$.
This only specifies $\Delta$ up to multiples of $4$, since $4 \tau^2 h_2 g$
is zero in the mANSS $E_2$-page.


    	
\begin{lem}
\label{q(Delta)}
Projection $q$ to the top cell takes
$\Delta$ to $-\tau \kappabar \cdot \nu$ or $-\tau \kappabar \cdot 5 \nu$.
\end{lem}

\cdan{One could choose $\nu$ to settle this ambiguity, but then there would
be a possible inconsistency with Bruner-Rognes's $\nu$.}

\begin{proof}
Because of the Adams-Novikov differential $d_5(\Delta) = \tau^2 h_2 g$
given in \cref{prop:d5_D},
\cref{topcell} implies that $q(\Delta)$ is detected by $-\tau h_2 g$.
Because of the presence of $\tau^2 h_1^3 g$ in higher filtration,
the element $-\tau h_2 g$ detects two homotopy elements
$-\tau \kappabar \cdot \nu$ and $-\tau \kappabar \cdot 5 \nu$.
\end{proof}

\begin{lem}
\label{nu0-detect}
The element $\nu_0$ is detected by $h_2$.
\end{lem}

\begin{proof}
From \cref{defn:nu_i}, we know that $q(\Delta) = - \tau \kappabar \cdot \nu_0$.
On the other hand, we also have the Adams-Novikov differential
$d_5(\Delta) = \tau^2 \Delta h_2 g$.
\cref{topcell} implies that $\tau \kappabar \cdot \nu$
is detected by $\tau \Delta h_2 g$.
It follows that $\nu_0$ is detected by $h_2$.
\end{proof}



\begin{lem}
\label{nu1-detect}
\mbox{}
\begin{enumerate}
\item
The element $\nu_1$ is detected by $2 \Delta h_2$.
\item
The element $\nu_5$ is detected by $2 \Delta^5 h_2$.
\end{enumerate}
\end{lem}

\begin{proof}
From \cref{defn:nu_i}, we know that $q(\Delta^2) = - \tau \kappabar \cdot \nu_1$.
On the other hand, we also have the Adams-Novikov differential
$d_5(\Delta^2) = 2 \tau^2 \Delta h_2 g$.
\cref{topcell} implies that $\tau \kappabar \cdot \nu_1$
is detected by $2 \tau \Delta h_2 g$.
It follows that $\nu_1$ is detected by $2 \Delta h_2$.

The proof of the second claim is nearly identical, using the formulas
$q(\Delta^6) = - \tau \kappabar \cdot \nu_5$ and
$d_5(\Delta^6) = 6 \tau^2 \Delta^5 h_2 g$.
The latter expression equals $2 \tau^2 \Delta^5 h_2 g$ because
$4 \Delta^2 h_2 g$ is zero in the mANSS $E_2$-page.
\end{proof}

\begin{lem}
\label{nu2-detect}
\mbox{}
\begin{enumerate}
\item
The element $\nu_2$ is detected by $3 \Delta^2 h_2$.
\item
The element $\nu_6$ is detected by $3 \Delta^6 h_2$.
\end{enumerate}
\end{lem}

\begin{proof}
From \cref{defn:nu_i}, we know that $q(\Delta^3) = - \tau \kappabar \cdot \nu_2$.
On the other hand, we also have the Adams-Novikov differential
$d_5(\Delta^3) = 3 \tau^2 \Delta^2 h_2 g$.
\cref{topcell} implies that $\tau \kappabar \cdot \nu_2$
is detected by $3 \tau \Delta h_2 g$.
It follows that $\nu_2$ is detected by $2 \Delta h_2$.

The proof of the second claim is nearly identical, using the formulas
$q(\Delta^7) = - \tau \kappabar \cdot \nu_6$ and
$d_5(\Delta^7) = 7 \tau^2 \Delta^6 h_2 g$.
The latter expression equals $3 \tau^2 \Delta^6 h_2 g$ because
$4 \Delta^6 h_2 g$ is zero in the mANSS $E_2$-page.
\end{proof}

\begin{lem}
\label{nu4-detect}
The element $\nu_4$ is detected by $\Delta^4 h_2$.
\end{lem}

\begin{proof}
From \cref{defn:nu_i}, we know that $q(\Delta^5) = - \tau \kappabar \cdot \nu_4$.
On the other hand, we also have the Adams-Novikov differential
$d_5(\Delta^5) = 5 \tau^2 \Delta^4 h_2 g$, which
equals $\tau^2 \Delta^4 h_2 g$ because $4 \Delta^4 h_2 g$ is zero
in the mANSS $E_2$-page.
\cref{topcell} implies that $\tau \kappabar \cdot \nu_4$
is detected by $\tau \Delta^4 h_2 g$.
It follows that $\nu_4$ is detected by $\Delta^4 h_2$.
\end{proof}

\begin{lem}
$\nu_2 \nu_4 = 3 \nu_0 \nu_6$.
\end{lem}

\begin{proof}
By \cref{nu_i-detect}, 
both products are detected by $\Delta^6 h_2^2$.
However, they are not necessarily equal because of the presence of
$\tau^4 \Delta^4 d g^2$ and $\tau^{10} \Delta^2 h_1^2 g^5$ in higher filtration.

We will show that $\tau \kappabar \cdot \nu_2 \nu_4$ equals
$\tau \kappabar \cdot 3 \nu_0 \nu_6$.
Our desired relation follows immediately because multiplication by
$\tau \kappabar$ is an isomorphism in the relevant degree.

We have
\[
q(\Delta^7 h_2) =  q(\Delta^3 \cdot \Delta^4 h_2) = 
q(\Delta^3 \cdot i(\nu_4)) = q(\Delta^3) \cdot \nu_4 = 
-\tau \kappabar \cdot \nu_2 \cdot \nu_4.
\]
Here we are using \cref{nu4-detect} to conclude that $i(\nu_4) = \Delta^4 h_2$.
On the other hand, we also have
\[
q(\Delta^7 h_2) = q(\Delta \cdot \Delta^6 h_2) =
q(\Delta \cdot i(3\nu_6) ) = q(\Delta) \cdot 3 \nu_6 =
- \tau \kappabar \cdot \nu_0 \cdot 3 \nu_6.
\]
Here we are using \cref{nu2-detect} to conclude that
$i(3\nu_6) = \Delta^6 h_2$.
\end{proof}

\begin{thm}
\label{nu4-nu6}
$\nu_4 \nu_6 = \nu_0 \nu_2 M$.
\end{thm}

\begin{proof}
By \cref{D4-M}, \cref{nu0-detect}, \cref{nu2-detect}, and \cref{nu4-detect}, 
both products are detected by $\Delta^{10} h_2^2$.
However, they are not necessarily equal because of the presence of
$\tau^4 \Delta^8 d g^2$ in higher filtration.

We will show that $\tau \kappabar \cdot \nu_4 \nu_6$ equals
$\tau \kappabar \cdot \nu_0 \nu_2 M$.
Our desired relation follows immediately because multiplication by
$\tau \kappabar$ is an isomorphism in the relevant degree.

We have
\[
q(3 \Delta^{11} h_2) = q(\Delta^5 \cdot 3 \Delta^6 h_2) =
q(\Delta^5 \cdot i(\nu_6)) = q(\Delta^5) \cdot \nu_6 =
-\tau \kappabar \cdot \nu_4 \cdot \nu_6.
\]
Here we are using \cref{nu2-detect} to conclude that
$i(\nu_6) = 3 \Delta^6 h_2$.
On the other hand, we also have
\[
q(3 \Delta^{11} h_2) = q(\Delta \cdot 3 \Delta^2 h_2 \cdot \Delta^8) =
q(\Delta \cdot i(\nu_2 \cdot M)) = q(\Delta) \cdot \nu_2 \cdot M =
- \tau \kappabar \cdot \nu_0 \cdot \nu_2 \cdot M.
\]
Here we are using \cref{D4-M} and \cref{nu2-detect} to conclude that
$i(\nu_2 \cdot M) = 3 \Delta^2 h_2 \cdot \Delta^8$.
\end{proof}

% Let $\alpha$ and $\beta$ be elements in $\pi_{*,*} \mmf$
% such that $\alpha$ is annihilated by $\tau$.  Then
% $\alpha$ is in the image of projection to the top cell, so
% $\alpha = q(a)$ for some element $a$ of $\pi_{*,*} \mmf/\tau$.
% Here we use the Roman symbol $a$ because
% $\pi_{*,*} \mmf/\tau$ is identified with the ANSS $E_2$-page.

% Now $\mmf/\tau$ is an $\mmf$-module, so
% $\pi_{*,*} \mmf/\tau$ is a $\pi_{*,*} \mmf$-module.
% In order to compute the action $a \cdot \beta$, 
% we can use that inclusion $i: \mmf \rightarrow \mmf/\tau$
% of the bottom cell is a ring map.  Therefore,
% \[
% a \cdot \beta = a \cdot i(\beta),
% \]
% where the second dot represents the product in the ANSS $E_2$-page.
% Note that $i(\beta)$ is zero when $\beta$ is divisible by
% $\tau$, and it equals an ANSS permanent cycle that detects $\beta$
% when $\beta$ is not divisible by $tau$.

% Next suppose that $k+1$ is congruent to $4$ modulo $8$.
% Using \cref{q-module-map}, 
% we have
% \begin{align*}
% & q( \tau \Delta^{j+k+1} h_1^3 ) =
% q(\Delta^{j+k+1} \cdot \tau h_1^3 ) =
% q (\Delta^{j+k+1} \cdot i( (k+1) \nu_0 )) = \\
% & = 
% q(\Delta^{j+k+1}) \cdot (k+1) \nu_0 =
% -\tau \kappabar \cdot \nu_{j+k} \cdot (k+1) \nu_0.
% \end{align*}
% Here we are using that $i(4 \nu_0) = \tau h_1^3$.  In other words,
% $4 \nu_0$ is detected by $\tau h_1^3$, which follows from the hidden
% $2$ extension from $2 h_2$ to $\tau h_1^3$ (see \cref{hidh0}).

% We will now compute $q( (k+1) \Delta^{j+k+1} h_2 )$ another way.
% We have $i(\nu_k) = (k+1) \Delta^k h_2$; in other words,
% $\nu_k$ is detected by the non-zero element $(k+1) \Delta^k h_2$,
% as shown in \cref{nu_i-detect}.  Then we have
% we have
% \[
% q( (k+1) \Delta^{j+k+1} h_2 ) = 
% q (\Delta^{j+1} \cdot (k+1) \Delta^k h_2) =
% q( \Delta^{j+1} \cdot i(\nu_k) ) = 
% q(\Delta^{j+1}) \cdot \nu_k =
% - \tau \kappabar \cdot \nu_j \cdot \nu_k.
% \]



% Finally, we must consider the case when $k+1$ is a multiple of $4$.
% In this case, 
% \[
% q( (k+1) \Delta^{j+k+1} h_2 ) = q(0) = 0.
% \]
% This implies that $(k+1) \nu_{j+k} \nu_0$ is zero.
% It suffices to observe that $\nu_j \nu_k$ is also zero.



% Finally, multiplication by $-\tau \kappabar$ is an isomorphism
% in the relevant degrees.

% The diagram
% \begin{equation}
% \label{eq:ASS}
% \xymatrix{
% \textrm{Adams $E_2$-page for $\mmf$} \ar[r] \ar@{=>}[d] & 
% \textrm{Adams $E_2$-page for $\mmf/\tau$} \ar@{=>}[d] \\
% \pi_{*,*} \mmf \ar[r] & \pi_{*,*} \mmf/\tau.
% }
% \end{equation}
% of Adams spectral sequences is induced by the inclusion
% $i: \mmf \rightarrow \mmf/\tau$ of the bottom cell.
% The lower right corner of the diagram is isomorphic to the
% Adams-Novikov $E_2$-page for $\mmf$, and 
% the Adams spectral sequence on the right side is isomorphic
% to the algebraic Novikov spectral sequence.



It turns out that all of the hidden extensions are preserved
by multiplication by $g$ and by $\Delta^8$.
In other words, assuming that $g x$ and $g y$ are non-zero, then
the following are equivalent:
\begin{enumerate}
\item 
there is a hidden $\alpha$ extension from $x$ to $y$.
\item 
there is a hidden $\alpha$ extension from $g x$ to $g y$.
\item
there is a hidden $\alpha$ extension from $\Delta^8 x$ to
$\Delta^8 y$.
\end{enumerate}
